GRAIL: Gradient-Based Adaptive Unlearning for Privacy and Copyright in LLMs

Large Language Models (LLMs) trained on extensive datasets often learn sensitive information, which raises significant social and legal concerns under principles such as the "Right to be forgotten." Retraining entire models from scratch to remove undesired information is both costly and impractical. Furthermore, existing single-domain unlearning methods fail to address multi-domain scenarios, where knowledge is interwoven across domains such as privacy and copyright, creating overlapping representations that lead to excessive knowledge removal or degraded performance. To tackle these issues, we propose GRAIL (GRadient-based AdaptIve unLearning), a novel multi-domain unlearning framework. GRAIL leverages gradient information from multiple domains to precisely distinguish the unlearning scope from the retention scope, and applies an adaptive parameter-wise localization strategy to selectively remove targeted knowledge while preserving critical parameters for each domain. Experimental results on unlearning benchmarks show that GRAIL achieves unlearning success on par with the existing approaches, while also demonstrating up to 17% stronger knowledge retention success compared to the previous state-of-art method. Our findings establish a new paradigm for effectively managing and regulating sensitive information in large-scale pre-trained language models.

==> table2_qwen_unlearn_two.tex <==
\begin{table*}[!t]
\caption{Experiments Results of unlearning Qwen-1.5-7B-Chat on User Privacy and Copyright}
\label{table:qwen_twocolumn}
\normalsize
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|c}
\toprule
\multirow{3}{*}{Models} & \multicolumn{6}{c|}{Privacy} & \multicolumn{6}{c|}{Copyright} &\multirow{2}{*}{Avg.} \\
\addlinespace[3pt]
\cline{2-13}
\addlinespace[3pt]
& \multicolumn{3}{c|}{Unlearn} & \multicolumn{3}{c|}{Retention} & \multicolumn{3}{c|}{Unlearn} & \multicolumn{3}{c|}{Retention} \\
\addlinespace[3pt]
\cline{2-14}
\addlinespace[3pt]
 & Succ $\uparrow$ & PPL $\uparrow$ & ROUGE-L $\downarrow$
 & Succ $\uparrow$ & PPL $\downarrow$ & ROUGE-L $\uparrow$
 & Succ $\uparrow$ & PPL $\uparrow$ & ROUGE-L $\downarrow$
 & Succ $\uparrow$ & PPL $\downarrow$ & ROUGE-L $\uparrow$ & Succ.$\uparrow$\\
 
\midrule
Vanilla Model & & & & & & & & & & & & & \\

\midrule
Gradient Ascent & & & & & & & & & & & & & \\
Fine-tuning with Random Labels & & & & & & & & & & & & & \\
Unlearning with adversarial samples & & & & & & & & & & & & & \\

\midrule
Gradient Ascent + Descent &  &  &  &  &  &  &  &  &  &  &  &  &\\
- Descent on in-distribution data & & & & & & & & & & & & & \\
- Descent on out-distribution data & & & & & & & & & & & & & \\
\midrule

Gradient Ascent + Descent &  &  &  &  &  &  &  &  &  &  &  &  &\\
- KL on in-distribution data & & & & & & & & & & & & & \\
- KL on out-distribution data & & & & & & & & & & & & & \\
\midrule

Memflex & & & & & & & & & & & & & \\
\midrule

AGU (Ours) & & & & & & & & & & & & & \\
\bottomrule
        
\end{tabular}
}
\end{table*}

==> table_llama_unlearn_HS.tex <==
\begin{table*}[t!]
\caption{Experiments Results of unlearning LLAMA-2-7B-Chat on User Privacy and Copyright} \vspace{-0.15cm}
\label{table1:unlearn_llama}
\normalsize
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|c|ccc|ccc|c|c}
\toprule

\multirow{3}{*}{Models} & \multicolumn{7}{c|}{Privacy} & \multicolumn{7}{c|}{Copyright} &\multirow{2}{*}{Avg.} \\

\addlinespace[3pt]
\cline{2-15}

\addlinespace[3pt]
& \multicolumn{3}{c|}{Unlearn} & \multicolumn{3}{c|}{Retention} & \multirow{1}{*}{} & \multicolumn{3}{c|}{Unlearn} & \multicolumn{3}{c|}{Retention} &\multicolumn{1}{c|}{}  \\ 
\addlinespace[3pt]
% \cline{2-7}
\cline{2-16}

\addlinespace[3pt]
 & Succ $\uparrow$ & PPL $\uparrow$ & ROUGE-L $\downarrow$ 
 & Succ $\uparrow$ & PPL $\downarrow$ & ROUGE-L $\uparrow$ & HS $\uparrow$
 & Succ $\uparrow$ & PPL $\uparrow$ & ROUGE-L $\downarrow$
 & Succ $\uparrow$ & PPL $\downarrow$ & ROUGE-L $\uparrow$ & HS $\uparrow$\\
 
\midrule
Vanilla Model & 0 & 1 & & 100 & & & & 0 & & & 100 & & & & \\

\midrule
Gradient Ascent & & & & & & & & & & & & & & \\
Fine-tuning with Random Labels & & & & & & & & & & & & & & \\
Unlearning with adversarial samples & & & & & & & & & & & & & & \\

\midrule
Gradient Ascent + Descent & & & & & & & & & & & & & & \\
- Descent on in-distribution data & & & & & & & & & & & & & & \\
- Descent on out-distribution data & & & & & & & & & & & & & \\
\midrule

Gradient Ascent + Descent & & & & & & & & & & & & & & \\
- KL on in-distribution data & & & & & & & & & & & & & & \\
- KL on out-distribution data & & & & & & & & & & & & & \\
\midrule

Memflex & 93.42 & & & 72.58 & & & & 100 & & & 80.04 & & & \\
\midrule

AGU (Ours) & \textbf{94.21} & & & \textbf{80.49} & & & & 100 & & & 81.16 & & & \\
\bottomrule
        
\end{tabular}
}
\end{table*}

%%\vspace{-0.2cm}

==> table_qwen_general.tex <==
\begin{table}[htb]
\caption{General task performance of QWEN-1.5-7B-CHAT after unlearning} \vspace{-0.15cm}
\label{table4:general_qwen}
\normalsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\toprule

\multirow{2}{*}{Models} & \multicolumn{6}{c}{General Task Performance} \\
\addlinespace[3pt]
\cline{2-7}
\addlinespace[3pt]
& MMLU & ARC & TruthfulQA & SIQA & RACE & Avg.\\

\addlinespace[3pt]
 
\midrule
Vanilla Model & 44.35 & 67.76 & 26.44 & 32.86 & 42.58 & 42.79 \\

\midrule
Gradient Ascent &  &  &  &  &  &\\
Fine-tuning with Random Labels & 43.04 & 63.51 & 29.62 & 32.65 & 36.84 & 41.13 \\
Unlearning with adversarial samples & 43.07 & 68.32 & 27.13 & 32.22 & 41.33 & 41.58\\

\midrule
Gradient Ascent + Descent & 43.04 & 63.51 & 29.62 & 32.65 & 36.84 & 41.13 \\
- Descent on in-distribution data & 44.04 & 60.69 & 28.02 & 33.00 & 41.72 & 41.49 \\
- Descent on out-distribution data & 41.97 & 65.59 & 25.94 & 32.80 & 40.00 & 41.54 \\
\midrule

Gradient Ascent + Descent &  &  &  &  &  &\\
- KL on in-distribution data & 43.45 & 56.69 & 24.47 & 33.31 & 28.51 & 37.29 \\
- KL on out-distribution data & 43.04 & 63.51 & 29.62 & 32.65 & 36.84 & 41.13 \\
\midrule

Memflex & 44.35 & 67.76 & 26.44 & 32.86 & 42.58 & 42.79 \\
\midrule

AGU (Ours) & 43.91 & 68.11 & 27.13 & 32.86 & 41.34 & 41.32 \\
w/o Gradient Localization & 43.41 & 68.22 & 28.13 & 32.13 & 41.30 & 41.21\\
w/o Adaptive Gradient Ascent + Descent & 43.07 & 68.32 & 27.13 & 32.22 & 41.33 & 41.58\\
\bottomrule
        
\end{tabular}
}
\end{table}

%%\vspace{-0.2cm}
